Can Small Language Models be Good Reasoners for Sequential Recommendation?

Large language models (LLMs) open up new horizons for sequential recommendations, owing to their remarkable language comprehension and generation capabilities. However, there are still numerous challenges that should be addressed to successfully implement sequential recommendations empowered by LLMs. Firstly, user behavior patterns are often complex, and relying solely on one-step reasoning from LLMs may lead to incorrect or task-irrelevant responses. Secondly, the prohibitively resource requirements of LLM (e.g., ChatGPT-175B) are overwhelmingly high and impractical for real sequential recommender systems. In this paper, we propose a novel Step-by-step knowLedge dIstillation fraMework for recommendation (SLIM), paving a promising path for sequential recommenders to enjoy the exceptional reasoning capabilities of LLMs in a "slim" (i.e., resource-efficient) manner. We introduce CoT prompting based on user behavior sequences for the larger teacher model. The rationales generated by the teacher model are then utilized as labels to distill the downstream smaller student model (e.g., LLaMA2-7B). In this way, the student model acquires the step-by-step reasoning capabilities in recommendation tasks. We encode the generated rationales from the student model into a dense vector, which empowers recommendation in both ID-based and ID-agnostic scenarios. Extensive experiments demonstrate the effectiveness of SLIM over state-of-the-art baselines, and further analysis showcasing its ability to generate meaningful recommendation reasoning at affordable costs.

==> backup/pre1008.tex <==
% \section{Preliminary \label{sec-pre}}

% Typically, a user's action sequence can be organized into a list ordered by timestamps $\mathcal{S}^{u}=\left\{S_1^{u}, S_2^{u}, \cdots, S_{t-1}^{u},\right\}$, 
% where $S_{k}^{u}$ represents an item clicked by user $u$ at time $k$ within the session.
% Let $\mathcal{I}=\left\{i_1, i_2, \cdots, i_M\right\}$ denote the set of $M$ items involved in all sessions, and $\mathcal{C}=$ $\left\{c_1, c_2, \cdots, c_R\right\}$ as the set of $R$ item attributes that express item characteristics,  such as title, category, brand, etc.
% Given a user session $\mathcal{S}^{u}$ and a candidate set of all possible items, our objective is to learn the representations of the user's session and all candidate items, 
% and then predict  $\hat{\textbf{y}}\in\{0, 1\}$  at time $t$,
% which each element in vector $\hat{\textbf{y}}$ indicates how likely this item should be recommended to the target user. 

\subsection{Sequential Recommendation Backbone \label{sec-pre}}
Sequential recommendation aims at the accurate prediction of user's next behavior by capturing evolved and dynamic preferences over historical behavior-sequences, which has occupied an critical position in various modern information systems~\cite{}.  In general, the success of sequential recommendation typically hings on the meaningful representation of items and effective encoding of behavior patterns. 

\paratitle{Item Representation}

\paratitle{Sequential Encoding}

\paratitle{Optimization}


In this work, we focus on the sequential recommendation task, which aims to capture the sequential characteristics of user behaviors for recommendation. 
Formally, given an item set $\mathcal{I}$, a user's action sequence can be organized in chronological order $\mathcal{S}_{u}=[i_1, i_2, \cdots, i_{t-1}]$, where $i_{k} \in \mathcal{I}$ represents the $k$-th item that the user $u$ interacted with, and each item $i$ is associated with several attributes, such as title, category, brand, etc. 
Based on the sequence $\mathcal{S}_{u}$, our objective is to predict the next item $i_t$ that the user $u$ is likely to interact with at the $t$-th step. 

In order to perform appropriate recommendation, mainstream neural recommendation methods learn the representations of the user's action sequence and candidate items, and then make predictions with the dot product of representations.
Typically, the action sequences and items can be encoded as sequential representation and item representation, respectively, as follows: 
\begin{equation}
    \begin{split}
        {z}^{\mathcal{S}_{u}} &= \operatorname{SeqEncoder}\left(\mathcal{S}_{u}\right), \nonumber \\
        {z}^{i} &= \operatorname{ItemEncoder}\left(i\right), \nonumber \\
    \end{split}
\end{equation}
where ${z}^{\mathcal{S}_{u}}$ and ${z}^{i}$ denote the representation of sequence $\mathcal{S}_{u}$ and item $i$, respectively. 
$\operatorname{SeqEncoder}$ and $\operatorname{ItemEncoder}$ can be sequence encoder and item encoder with arbitrary architecture. 
Base on the above representations, we can obtain the final prediction  $\hat{\textbf{y}}\in\{0, 1\}$  at time $t$, where each element $\hat{\textbf{y}}_{ui}$ indicates how likely the item $i$ should be recommended to the target user $u$. 
Finally, the recommendation model can be trained with Binary Cross-Entropy (BCE)~\cite{} loss as follows:
\begin{equation}
    \mathcal L \!=\! - \sum_{u \in \mathcal{U}}\sum_{i \in \mathcal{I}} 
    {\textbf{y}}_{ui} \log \hat{\textbf{y}}_{ui} 
    + (1-\textbf{y}_{ui}) \log \left(1-\hat{\textbf{y}}_{ui}\right). \nonumber \\
\end{equation}

Note that these classical sequencical models typically perform recommendation based on the user action sequences and item attributes (\emph{e.g.,} title, category and brand), overlooking the CoT power of large language models that have emerged recently.






